WDiscOOD: Out-of-Distribution Detection via Whitened Linear Discriminant Analysis

Deep neural networks are susceptible to generating overconfident yet erroneous predictions when presented with data beyond known concepts. This challenge underscores the importance of detecting out-of-distribution (OOD) samples in the open world. In this work, we propose a novel feature-space OOD detection score based on class-specific and class-agnostic information. Specifically, the approach utilizes Whitened Linear Discriminant Analysis to project features into two subspaces - the discriminative and residual subspaces - for which the in-distribution (ID) classes are maximally separated and closely clustered, respectively. The OOD score is then determined by combining the deviation from the input data to the ID pattern in both subspaces. The efficacy of our method, named WDiscOOD, is verified on the large-scale ImageNet-1k benchmark, with six OOD datasets that cover a variety of distribution shifts. WDiscOOD demonstrates superior performance on deep classifiers with diverse backbone architectures, including CNN and vision transformer. Furthermore, we also show that WDiscOOD more effectively detects novel concepts in representation spaces trained with contrastive objectives, including supervised contrastive loss and multi-modality contrastive loss.

==> tables/res50_results.tex <==
\begin{table*}
    \centering
    \setlength\tabcolsep{2.5 pt}
%    \begin{tabular}{@{}l@{}llc@{}lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}}
%	\begin{tabular}{@{} l @{} lc@{} lc@{} lc@{} lc@{} lc@{} lc@{} lc@{}}
	\begin{tabular}{@{}l @{} l c@{}c c@{}c c@{}c c@{}c c@{}c c@{}c c@{}c c@{}c}
        \toprule
%        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Model}\end{tabular}}
         & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Method}\end{tabular}} 
%         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Source}\end{tabular}} 
         & \multicolumn{2}{c}{\textbf{Textures}} 
         & \multicolumn{2}{c}{\textbf{SUN}} 
         & \multicolumn{2}{c}{\textbf{Places}} 
         & \multicolumn{2}{c}{\textbf{iNaturalist}} 
         & \multicolumn{2}{c}{\textbf{ImgNet-O}} 
         & \multicolumn{2}{c}{\textbf{OpenImg-O}} 
         & \multicolumn{2}{c}{\textbf{Average}}                                                                                                                                                        \\
         &  & {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	\\
        \cmidrule(r){1-2} \cmidrule(lr){3-14} \cmidrule{15-16}
%        \multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}BiT\end{tabular}}
		 & \multicolumn{15}{c}{\textbf{Classifier-dependent methods}}  \\
         & {MSP}~\cite{msp} 
%         		& prob 
         		& $72.98$ & $74.92$
         		& $70.98$ & $78.75$ 
         		& $\underline{73.43}$ & $76.65$
         		& $60.90$ & $84.40$ 
         		& $95.65$ & $53.13$   
         		& $69.73$ & $81.17$
         		& $73.94$ & $74.84$
         		\\
         & {Energy}~\cite{energyOOD} 
%         		& logit 
         		& $95.74$ &  $48.60$
         		& $97.93$ &  $50.12$
         		& $97.77$ &  $48.90$
         		& $98.12$ &  $50.86$
         		& $92.80$ &  $48.23$
         		& $95.41$ &  $52.33$
         		& $96.30$ &  $49.84$
         		\\
         & {ODIN}~\cite{odin} 
%         		& prob+grad 
         		& $75.94$ &  $69.33$
         		& $75.51$ &  $74.05$
         		& $77.54$ &  $71.28$
         		& $68.60$ &  $79.88$
         		& $94.95$ &  $51.19$
         		& $73.98$ &  $76.15$
         		& $77.75$ &  $70.31$
         		\\
         & {MaxLogit}~\cite{maxlogit}     
%         		& logit 
         		& $75.92$ & $69.33$  
         		& $75.51$ & $74.05$
         		& $77.55$ & $71.28$
         		& $68.57$ & $79.88$
         		& $94.95$ & $51.19$
         		& $73.97$ & $76.15$
         		& $77.74$ & $70.31$
         		\\
         & {KLMatch}~\cite{maxlogit}  
%         		& prob  
         		& $57.57$ & $86.09$
         		& $70.36$ & $\underline{82.91}$
         		& $\underline{74.04}$ & $\underline{80.65}$
         		& $46.83$ & $90.81$
         		& $89.75$ & $68.86$
         		& $58.21$ & $88.31$
         		& $66.13$ & $82.94$
         		\\
         & {ReAct}~\cite{react} 
%         		& feat+logit 
         		& $98.05$ & $34.51$
         		& $99.66$ & $23.68$
         		& $99.80$ & $22.86$
         		& $100.00$ & $23.13$
         		& $99.40$ & $37.31$
         		& $99.86$ & $23.86$
         		& $99.46$ & $27.56$
         		\\
         & {ViM \cite{vim}} 
%         		& feat+logit 
         		& $\underline{25.18}$ & $\underline{92.63}$
         		& $\underline{69.22}$ & $81.39$
         		& $74.90$ & $76.40$
         		& $\underline{30.02}$ & $\underline{93.38}$
         		& $\underline{76.15}$ & $\underline{77.08}$ 
         		& $\underline{46.70}$ & $\underline{88.60}$
         		& $\underline{53.70}$ & $\underline{84.91}$
         		\\
         \cmidrule(r){1-2} \cmidrule(lr){3-14} \cmidrule{15-16}
         & \multicolumn{15}{c}{\textbf{Feature space methods}}  \\
%         & {Residual \cite{vim}} 
%%         		& feat
%         	 	& $28.10$ & $92.04$
%         		& $72.49$ & $80.35$
%         		& $77.89$ & $75.67$
%         		& $34.05$ & $92.45$
%         		& $76.40$ & $76.29$
%         		& $51.41$ & $87.24$
%         		& $56.72$ & $84.01$
%         		\\
         & {Maha}~\cite{mahaOOD} 
%         		& feat+label
         		& $31.17$ & $91.62$ 
         		& $\underline{66.29}$ & $\underline{84.31}$ 
         		& $\underline{70.27}$ & $\underline{81.45}$
         		& $\underline{25.64}$ & $\underline{95.38}$
         		& $81.45$ & $75.65$ 
         		& $\bm{44.36}$ & $\bm{91.41}$ 
         		& $\underline{53.20}$ & $\underline{86.64}$
         		\\
         & {KNN~\cite{knnOOD}} 
%         		& feat
         	 	& $\bm{23.26}$ & $\bm{93.11}$
         	 	& $88.59$ & $74.01$
         	 	& $89.00$ & $71.07$
         	 	& $74.60$ & $85.83$
         	 	& $\bm{71.05}$ & $\bm{81.15}$ 
         	 	& $70.29$ & $84.01$
         	 	& $69.47$ & $81.53$
          	 	\\
         & {\textbf{\methName}}
         		& $\underline{29.20}$ & $\underline{91.90}$
         		& $\bm{56.83}$ & $\bm{86.74}$
         		& $\bm{64.40}$ & $\bm{83.13}$
         		& $\bm{22.39}$ & $\bm{95.59}$ 
         		& $81.60$ & $75.52$
         		& $\underline{44.67}$ &	$\underline{90.51}$
         		& $\bm{49.85}$ & $\bm{87.23}$
         		\\
%        \cmidrule(r){1-3}\cmidrule(lr){4-11}\cmidrule(l){12-13}
%        \multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}ViT\end{tabular}} \\
        \bottomrule
    \end{tabular}
    \caption{
        \textbf{Results on ResNet-50\cite{resnet} classification model}. 
        We test all methods on six OOD datasets and compute the average performance.
        Both metrics AUROC and FPR95 are in percentage.
        We highlight the best performance in bold, and underline the 2nd and 3rd ones.
%        The rows are organized in ascend order according to average AUROC.
%        \red{I just cannot get good result for Energy as others. The implementation should be correct as its performance on ViT is very strong.}
    }\label{tab:res50Clf}
\end{table*}


==> tables/vit_results.tex <==
\begin{table*}
    \centering
    \setlength\tabcolsep{2.5 pt}
%    \begin{tabular}{@{}l@{}llc@{}lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}}
%	\begin{tabular}{@{} l @{} lc@{} lc@{} lc@{} lc@{} lc@{} lc@{} lc@{}}
	\begin{tabular}{@{}l @{} l c@{}c c@{}c c@{}c c@{}c c@{}c c@{}c c@{}c c@{}c}
        \toprule
%        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Model}\end{tabular}}
         & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Method}\end{tabular}} 
%         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Source}\end{tabular}} 
         & \multicolumn{2}{c}{\textbf{Textures}} 
         & \multicolumn{2}{c}{\textbf{SUN}} 
         & \multicolumn{2}{c}{\textbf{Places}} 
         & \multicolumn{2}{c}{\textbf{iNaturalist}} 
         & \multicolumn{2}{c}{\textbf{ImgNet-O}} 
         & \multicolumn{2}{c}{\textbf{OpenImg-O}} 
         & \multicolumn{2}{c}{\textbf{Average}}                                                                                                                                                        \\
         &  & {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	& {\footnotesize FPR95$\downarrow$} & {\footnotesize AUROC$\uparrow$}
         	\\
        \cmidrule(r){1-2} \cmidrule(lr){3-14} \cmidrule{15-16}
%        \multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}BiT\end{tabular}}
		 & \multicolumn{15}{c}{\textbf{Classifier-dependent methods}}  \\
         & {MSP}~\cite{msp} 
%         		& prob 
         		& $52.43$ & $85.42$
         		& $53.22$ & $86.93$ 
         		& $57.75$ & $85.72$
         		& $13.66$ & $97.00$ 
         		& $51.75$ & $85.81$   
         		& $31.99$ & $92.48$
         		& $43.47$ & $88.89$
         		\\
         & {Energy}~\cite{energyOOD} 
%         		& logit 
         		& $36.13$ & $91.25$
         		& $\underline{34.44}$ & $\underline{93.28}$
         		& $\bm{42.80}$ & $\bm{90.98}$
         		& $5.60$ &  $98.94$
         		& $\underline{30.30}$ & $93.36$
         		& $16.06$ & $96.87$
         		& $27.56$ & $94.11$
         		\\
         & {ODIN}~\cite{odin} 
%         		& prob+grad 
         		& $38.56$ &  $90.86$
         		& $37.45$ &  $92.81$
         		& $44.68$ &  $\underline{90.66}$
         		& $6.03$ &   $98.81$
         		& $33.50$ &  $92.69$
         		& $17.83$ &  $96.54$
         		& $29.68$ &  $93.73$
         		\\
         & {MaxLogit}~\cite{maxlogit}     
%         		& logit 
         		& $38.56$ & $90.86$
         		& $37.45$ & $92.81$
         		& $44.68$ & $\underline{90.66}$
         		& $6.03$ &  $98.81$
         		& $33.50$ & $92.69$
         		& $17.83$ & $96.54$
         		& $29.68$ & $93.73$
         		\\
         & {KLMatch}~\cite{maxlogit}  
%         		& prob  
         		& $51.22$ & $85.12$
         		& $56.04$ & $85.45$
         		& $61.08$ & $83.86$
         		& $13.68$ & $96.32$
         		& $49.90$ & $85.62$
         		& $31.38$ & $91.93$
         		& $43.88$ & $88.05$
         		\\
         & {ReAct}~\cite{react} 
%         		& feat+logit 
         		& $\bm{36.35}$ &  $91.17$
         		& $34.55$ &  $93.22$
         		& $\underline{43.32}$ &  $\underline{90.83}$
         		& $5.61$ &   $98.94$
         		& $\underline{30.30}$ &  $93.40$
         		& $\underline{16.01}$ &  $96.88$
         		& $27.69$ &  $94.07$
         		\\
         & {ViM \cite{vim}} 
%         		& feat+logit 
         		& $38.67$ & $\underline{91.38}$
         		& $\bm{32.47}$ & $\bm{93.41}$
         		& $44.23$ & $89.86$
         		& $\underline{1.40}$ & $\underline{99.68}$
         		& $31.80$ & $\underline{94.05}$ 
         		& $16.61$ & $\underline{97.10}$
         		& $\underline{27.53}$ & $\underline{94.25}$
         		\\
         \cmidrule(r){1-2} \cmidrule(lr){3-14} \cmidrule{15-16}
         & \multicolumn{15}{c}{\textbf{Feature space methods}}  \\
%         & {Residual \cite{vim}} 
%%         		& feat
%         	 	& $49.06$ & $89.35$
%         		& $38.63$ & $91.29$
%         		& $52.81$ & $86.56$
%         		& $1.51$ & $99.62$
%         		& $40.10$ & $92.21$
%         		& $25.41$ & $95.58$
%         		& $34.59$ & $92.44$
%         		\\
         & {Maha}~\cite{mahaOOD} 
%         		& feat+label
         		& $\underline{36.61}$ & $\underline{91.67}$ 
         		& $35.37$ & $92.89$ 
         		& $46.08$ & $89.55$
         		& $\underline{0.96}$ & $\underline{99.78}$
         		& $30.45$ & $\underline{94.22}$ 
         		& $\bm{13.85}$ & $\bm{97.50}$ 
         		& $\underline{27.22}$ & $\underline{94.27}$
         		\\
         & {KNN~\cite{knnOOD}} 
%         		& feat
         	 	& $38.28$ & $90.74$
         	 	& $46.08$ & $90.73$
         	 	& $54.50$ & $87.54$
         	 	& $6.75$ & $98.70$
         	 	& $38.95$ & $92.53$ 
         	 	& $20.59$ & $96.12$
         	 	& $34.19$ & $92.72$
          	 	\\
         & {\textbf{\methName}}
         		& $\underline{36.58}$ & $\bm{91.79}$
         		& $\underline{32.62}$ & $\underline{93.34}$
         		& $\underline{43.74}$ & $89.91$
         		& $\bm{0.89}$ & $\bm{99.81}$ 
         		& $\bm{30.15}$ & $\bm{94.36}$
         		& $\underline{14.30}$ & $\underline{97.44}$
         		& $\bm{26.38}$ & $\bm{94.44}$
         		\\
%        \cmidrule(r){1-3}\cmidrule(lr){4-11}\cmidrule(l){12-13}
%        \multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}ViT\end{tabular}} \\
        \bottomrule
    \end{tabular}
    \caption{
        \textbf{Results for ViT-B/16\cite{ViT} classification model}. 
        We test all methods on six OOD datasets and compute the average performance.
        Both metrics AUROC and FPR95 are in percentage.
        We highlight the best performance in bold, and underline the 2nd and 3rd ones.
%        The rows are organized in ascend order according to average AUROC. 
    }\label{tab:vitClf}
\end{table*}

